Edge-Aided Sensor Data Sharing in Vehicular Communication Networks

Sensor data sharing in vehicular networks can significantly improve the range and accuracy of environmental perception for connected automated vehicles. Different concepts and schemes for dissemination and fusion of sensor data have been developed. It is common to these schemes that measurement errors of the sensors impair the perception quality and can result in road traffic accidents. Specifically, when the measurement error from the sensors (also referred as measurement noise) is unknown and time varying, the performance of the data fusion process is restricted, which represents a major challenge in the calibration of sensors. In this paper, we consider sensor data sharing and fusion in a vehicular network with both, vehicle-to-infrastructure and vehicle-to-vehicle communication. We propose a method, named Bidirectional Feedback Noise Estimation (BiFNoE), in which an edge server collects and caches sensor measurement data from vehicles. The edge estimates the noise and the targets alternately in double dynamic sliding time windows and enhances the distributed cooperative environment sensing at each vehicle with low communication costs. We evaluate the proposed algorithm and data dissemination strategy in an application scenario by simulation and show that the perception accuracy is on average improved by around 80 % with only 12 kbps uplink and 28 kbps downlink bandwidth.

==> Sections/1_introduction.tex <==
\section{Introduction}

\Caf{\emph{PLS DO NOT CHANGE ANYTHING IN SEC I INTRO, I AM WORKING ON IT. }}

\emph{Cooperative Perception} CP enables \emph{Connected Automated Vehicles} (CAV) to acquire %more sufficient and 
accurate environmental information by sharing their locally perceived sensor data via communication, and thereby improving the safety and efficiency in road traffic. % system.
%Due to the limited communication resource in network, 
In order to reduce the data load in the resource-constrained communication network, 
%and the computation abilities in \emph{On-Board Unit} (OBU)
the perception information is rather shared as list of detected and classified objects than as raw sensor data. Subsequently, the cooperative perception can be realized by
%results can be \Caf{developed ?} \Crs{(deduced?)} 
% using 
object level data fusion either in a distributed or a centralized fashion. 
Previous work \cite{schiegg2021}, \cite{FISITA2021} evaluated and summarized existing approaches for sensor data sharing in %C-ITS 
vehicular networks. To acquire a better estimation of the states of a target vehicle, e.g. its position and velocity, based on cooperative perception information \cite{8916837}, \cite{Shorinwa2020}, \cite{zhang2021distributed} investigated data fusion methods in the Vehicle-to-Everything (V2X) environment. However, the perception measurement quality, which is normally characterized as measurement noise, in each CAV is always unknown while CP, which leads to failures in sensor fusion results in V2X. 
Only little research has been carried out to determine how to cooperatively estimate the measurement noise in V2X. Although the concept of transmitting the quality of sensor data is under discussion, the measurement noise in each CAV can be unexpected changed, due to effects from road and weather conditions, individual wearing of hardware, diverse combinations of sensor types, bias in training data, etc. Also, the information about inaccuracy of CAVs may not be shared because of the sensitivity and privacy.
%Thus, we believe the perception accuracy in each vehicle is usually unknown and hence hard to be direct transmitted in V2X messages. 

%However, the quality of the shared sensor data from each CAV in the network is individual and usually unknown. \Cah{Although} the sensors can be calibrated, the measurement noise is varied by road and weather conditions, wearing of hardware, bias in training data, etc. 
%Therefore, how to \Cah{weigh} the sensor measurement from local On-Board Sensor (OBS) and foreign CAVs is crucial for the CP. 

\begin{figure}[b]
   \centering
   \includegraphics[width=0.4\textwidth]{figures/intro_of_system.png}
   \caption{Sensor data sharing by means of vehicle-to-cloud (V2C) and vehicle-to-vehicle (V2V) communications in vehicular networks composed of an edge server and an associated vehicle fleet, including CAVs and normal vehicles}
   \label{fig:system}
\end{figure}

\Crs{The sensor data sharing in vehicular networks with an edge server is shown in Fig.~\ref{fig:system}.} Although the centralized data fusion at the edge server that is connected with all CAVs in a dedicated area, i.e. vehicle fleet, provides better perception results comparing distributed data fusion in each CAV, the sensor measurement noise in single CAV can cause heavy errors. Moreover, directly transmitting the centralized fusion results from Edge to vehicles requires latency in millisecond level that is hard to achieve. 
%Thus, acquiring noise knowledge for each CAV is  essential for distributed data fusion results.
Thus, we believe the noise estimation for distributed data fusion in each CAV is necessary and essential for CP success.

In this paper, we attempt to estimate the sensor measurement noise in each CAV at a computation center, i.e., an edge server. This server is capable to share the noise knowledge to all CAVs in a vehicle fleet and to enhance the distributed object-level sensor data fusion. The key contributions are:

\begin{itemize}
    \item Pointing out the problem with unknown noise values in cooperative perception by sharing sensor data in V2X.
    \item Developing the BiFNoE algorithm that determines the noise estimations for each CAV and improves the centralized target estimation at an edge server.
    \item Proposing a system with a noise estimation service, which enhances the distributed estimation at a single CAV.
    \item Providing a thorough empirical evaluation and investigating the trade-off between perception accuracy and communication costs.% and using our system.
    \item Implementing the BiFNoE algorithm and the proposed system in a simulation environment and validating the feasibility of the proposed approach in an urban scenario. % with significant performance metrics. 
    The open-source code is available at: \Crs{Github link?}
\end{itemize}

%%%%%%%%commented%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}
    \item Pointing out the noise problem in the partially connected vehicle fleet and developing the BiFNoE algorithm that iteratively estimates the noise and targets based on sensor data sharing in V2N communication.
    \item  Proposing a system with noise estimation service, which enhances the distributed estimation at single vehicle.
    \item  Providing a thorough empirical evaluation and investigating the trade-off between limited communication resource and perception quality using our proposed protocol.
    \item  Implementing the algorithm and protocol in CARLA simulator and validating the feasibility in an urban scenario with significant performance metrics. The open-source code is available at: \Crs{Github link?}
\end{itemize}
\end{comment}
%%%%%%%%commented%%%%%%%%%%%%%%%

The remainder of this paper is structured as follows. Section~\ref{sec:related_work} summarizes related work in sensor data sharing fusion in V2X network. The problem with unknown noise values in a multi-agent system is formulated in Section~\ref{sec:problem_formulation}. The algorithm for noise estimation is introduced in Section~\ref{sec:algorithm} and the associated system is proposed in Section~\ref{sec:protocol}. The performance of algorithm and protocol is comprehensively evaluated in Section~\ref{sec:evaluation} considering communication costs.  Section~\ref{sec:conclusion} provides a summary and concludes. 



==> Sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

 \Cah{A first approach to distributed state estimation in sensor networks has been carried out in~\cite{wang2018}. Although in large-scale sensor networks, some global parameters can be learnt offline, it is still possible that these parameters change with time due to various factors such as sensor failures, problems in communication channels etc. This in turn deteriorates the performance of local parameters. The approach in~\cite{wang2018}, carefully considers the time varying nature of the sensing models and arrives at a consistent distributed sensor state estimation technique. %AF: Here, you introduce 'global' and 'local' parameters, which is rather unclear at this stage. Also, it is really the case that cite{wang2018} is "a first approach"? Hard to believe because it is rather new (from 2018). Finally, here you start talking about sensor networks, but the intro is about V2X (I of course know that there are similarities, but it is obvious.)
 
 The significance of distributed kalman filtering (DKF) for sensor networks has been studied in~\cite{Olfati2005}. The author addressed the DKF problem by reducing it to two separate dynamic consensus problems in terms of weighted measurements and inverse-covariance matrices and solved them by employing two types of consensus filters.
 
 The challenges of centralized estimation approaches to target tracking in autonomous vehicle fleets have been studied in~\cite{Shorinwa2020}. The authors have proposed a scalable Distributed Rolling Window Tracking (DRWT) algorithm, which addresses the problem of distributed target tracking in a fleet of vehicles collaborating over a dynamic communication network. This approach has proven to show equivalent performance to the classical consensus kalman filtering techniques as highlighted in \cite{Olfati2005}.}

\Crs{Paragraphs for noise are needed. More literature in Reference are needed}

\Caf{This section should also summarize the main commonalities and differences of your paper in comparison to the literature.}
 
 \Crs{Sensor fusion in V2X - Noise in sensor fusion - conventional noise estimation - comparison with our method}
 %The idea has been inspired by (not only) the following papers:
 %\cite{Shorinwa2020}
 %\cite{FISITA2021}
 %\cite{7979571}
 %\cite{HE202021}
 %\cite{Olfati2005}
 %\cite{zhang2021distributed}
 %\cite{Wang2020}
 %Sensor Data sharing (vehicle fleet, edge, sharing frameworks) and fusion (fusion in object level, centralized and distributed Kalman Filter)
 
 % Study on Noise in sensor network
 



==> Sections/2_related_work_v2.tex <==
 \section{Related Work}
\label{sec:related_work}

 %Sensor sharing and fusionusion accomplish CP in vehicular network, where distributed estimation method is the key approach, especially for fusing the shared data in object level. 
 % Proposal:
Environmental perception is commonly regarded as a major challenge for the realization of vehicle automation. Sensor data sharing among vehicles helps increasing the range and the accuracy of perception. 
%%%%%%From Introduction
Previous work on sensor data sharing has primarily studied the data dissemination in the context of vehicular communication for ad hoc networks, see %e.g.,~\cite{Delooz2020,Garlich2019,Thandavarayan2020,schiegg2021}, %%%%%
e.g.,~\cite{Delooz2020,Thandavarayan2020,schiegg2021}, and for vehicle-to-cloud communication~\cite{FISITA2021}. Sensor data sharing is also being considered in the standardization processes of vehicular communication~\cite{ETSI-TR103562-CPS-studyitem,SAE_CP}. To acquire a better estimation of the states of a target vehicle, e.g., its position and velocity, based on sensor data sharing, %\cite{8916837,Shorinwa2020,zhang2021distributed}%%%%%
\cite{Shorinwa2020,zhang2021distributed} investigated data fusion methods.
%%%%% From Introduction

Among the wide spectrum of existing work in the area of sensor data sharing and fusion<, the distributed estimation method is a key approach, especially for the fusion of shared data at object level. %
By applying consensus-based Kalman Filter methods~\cite{5399678},
%\cite{Olfati2005,5399678,BATTISTELLI2016169},
a CAV is able to aggregate the perceived information from on-board sensors and from all other CAVs in the communication range, thereby improving the state estimation of the target vehicles. Several distributed estimation strategies and protocols have been proposed, %e.g., in~\cite{5411741,yuan2017distributed,SHIN2020259,9204471},%%%%%
e.g., in~\cite{5411741,yuan2017distributed,9204471}, where only a finite number of measurements from reachable nodes is taken into account. In~\cite{HE202021}, these publications were summarized and compared by simulations in terms of global optimality, local consistency, communication overhead 
 and topology requirements.

In vehicular applications and others, the sensors' measurement noise in each CAVs, which is unknown and time-varying, can cause a bad estimation. The existing methods for handling the noise  aim either at the use of advanced statistical models~\cite{9195416,8036249,8326722}
or at a better calibration process as part of the manufacturing process. Both methods are not suitable for the sensor data fusion in vehicular scenarios. The reasons are:
\begin{itemize}
    \item %Dynamic
    The measurement providers are only temporary reachable CAVs in the vehicular network.
    \item %Dependency: 
    The measurement inaccuracy depends on the environmental conditions, e.g. road, weather, lighting, etc.
    \item %Bias: 
    The performance of AI-based measurements, i.e., detection results, can be affected by the bias in training data.
\end{itemize}
While state-of-the-art for automatic calibration using camera~\cite{6909022,10.1145/3199667}, LiDAR~\cite{9010134,8317829} or hybrid sensor combinations~\cite{8917135} can provide the knowledge about inaccuracy of the on board sensors' detection a vehicle, but requires an additional advanced sensor set-up in roadside units. Moreover, the potential detection failures in roadside units can affect the quality for each CAV implementing the automatic calibration. 

%Will the following paragraph be transferred to the first section?
In this paper, we address those challenges in vehicular applications and employ a novel approach to the problem of noise estimation. We apply the %centralized and distributed 
estimation in continuously available edge servers and CAVs in a dedicated vehicle fleet, where the CAVs can upload their sensor data to the edge server. Compared to the automatic calibration approaches, our proposed solution does not require an additional sensor setup. Instead, we optimize the noise estimation in double dynamic sliding time windows at the edge server. 
By subscribing the proposed noise estimation service, the CAVs improve their estimations, which converge to the limit.
 

==> Sections/6_evaluation.tex <==
\section{Simulation Results}
\label{sec:evaluation}
\subsection{Algorithm Evaluation}

\begin{figure*}[ht]
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/BiFNoE_v2.png}
\caption{Centralized noise and target estimation (est.) using BiFNoE. We observe the BiFNoE performance under different sensor data uploading frequency, 50\,Hz, 10\,Hz, 1\,Hz and 0.25\,Hz in four columns. The centralized noise and target estimation accuracy is characterized by the mean squared error to ground truth (gt.) in the first two rows. We consider the noise estimation with target ground truth and target estimation with noise ground truth alternately as the limit. The last row shows the BiFNoE forced centralized target estimation to converge to the limit. The convergence speed is increased with the rising uploading frequency.}
\label{fig:BiFNoE}
\end{figure*}

The algorithm is evaluated first in a simulation with N\,=\,100 CAVs and M\,=\,100 normal vehicles. Each CAV is able to detect the position of moving objects in its individual detection range, which is randomly generated within $[100:300]~m$. The diagonal of the covariance matrix $R_i$ for each vehicle is randomly set within $[0.01^2:5^2]~m^2$ in the initializing phase. Local perception results in form of object list $\mathcal{D}_{i,t}$ with registered ID and position are broadcasted to the neighbor CAVs within a communication range 150\,m and uploaded to the edge server. The simulation tick frequency $f_{sim} = 50\,Hz$ is the same as the broadcast frequency $f_{bdc}$ for data sharing in self-managed network, while the upload frequency $f_{upl}$ is usually lower and can be varied.



%%%%%%commented%%%%%%
\begin{comment}
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{0.49\textwidth}
   \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/ckf_target_est_1.PNG}
   \caption{\centering Centralized estimation with predefined noise value (red), learned noise values (blue) and noise ground truth (black) with respect to the target ground truth}
   \label{fig:ckf_target_est_1} 
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
   \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/ckf_target_est_2.PNG}
   \caption{\centering Centralized estimation with predefined noise value (red), learned noise values (blue) with respect to the estimation limit, i.e., estimation with noise ground truth}
   \label{fig:ckf_target_est_2}
\end{subfigure}
\caption{\centering Centralized estimation with and without noise learning}
\label{fig:ckf_target_est}
\end{figure*}
\end{comment}
%%%%%%commented%%%%%%

The centralized noise and target estimation using BiFNoE are shown in Fig.~\ref{fig:BiFNoE}. 
The first row depicts the MSE of the noise estimation with different sensor data upload frequency $f_{upl}$ with respect to the noise ground truth of each CAV. With an increasing iterative stage number in time series, the noise estimation approaches to the theoretical limit of the algorithm, where the ground truth of target $x_{c,l,\tau}$ instead of $\hat{x}_{c,l,\tau}$ is used 
%in the setup of \Caf{{Update Noises in Time Window II} ?}.
as mean of noise model for noise estimation in time window II. 

It is clear that the lower $f_{upl}$ reduces the convergence speed because of the less implementation number of BiFNoE within the same time slots. However, the accuracy of centralized target estimation can still be visible increased comparing with the estimation without BiFNoE, as shown in second row. The bidirectional feedback enables the convergence speed of centralized target estimation almost the same as it in noise estimation. The MSE of target estimation with respect to the target estimation limit is emphasized in the third row. It shows that the accuracy of centralized target estimation can be notable increased and close to the limit by running BiFNoE at edge server

%Only with a default $\hat{R}_{i,0}$ with diagonal of $0.01^2$, the \emph{Mean Squared Error} (MSE) of the target estimation is around 1\,m (Figure~\ref{fig:ckf_target_est_1}). The \ref{alg:BiFNoE} algorithm improves the MSE of the estimation to about 0.02\,m after 2\,s with a high convergence speed thanks \Caf{to fast increasing data} in the edge server. To show the limit of the estimation enhanced by noise learning, the target states are \Caf{meanwhile ?} estimated based on the noise ground truth $R_i$. We  can observe in Figure~\ref{fig:ckf_target_est_2} that the estimation always follows the limit based on $\hat{R}_{i,t}$ stably and closely, compared to the centralized estimation only based on the default $\hat{R}_{i,0}$.

%%%%%%commented%%%%%%
\begin{comment}
\begin{figure}[ht]
\includegraphics[width=.49\textwidth]{figures/noise_est.PNG}
\caption{Noise Estimation}
\label{fig:noise_est}
\end{figure}
\end{comment}
%%%%%%commented%%%%%%

\begin{figure*}[ht]
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/dkf_res_v3.png}
\caption{Distributed estimation enhanced by BiFNoE. We consider the scenarios with different communication range 150\,m, 80\,m and 0\,m in three columns, where 0\,m corresponds to the case of no communication in the  ad hoc network, where only local sensor data used used to estimate the targets detected. We compared the mean squared errors to the ground truth distributed estimation with subscription frequency of 10\,Hz, 1\,Hz and 0\,Hz (no subscription) in the first row and the mean squared errors to the estimation limit, where the noise ground truth is used for distributed estimation in the second row. The low-frequency subscription can still ensure that the distributed estimation converges to its limit. }
\label{fig:dist_est}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/dst_target_est_1.PNG}
   \caption{\centering Distributed estimation with predefined noise value (red), learned noise values (blue) and noise ground truth (black) with respect to the target ground truth}
   \label{fig:dst_target_est_1} 
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/dst_target_est_2.PNG}
   \caption{\centering Distributed estimation with predefined noise value (red), learned noise values (blue) with respect to estimation limit, i.e. estimation with noise ground truth}
   \label{fig:dst_target_est_2}
\end{subfigure}
\caption{\centering Distributed Estimation with and without Noise Learning}
\label{fig:dst_target_est}
\end{figure*}

\subsection{System Evaluation}

When the estimated noise values are transmitted as messages to each CAV in this vehicle fleet. The augmentation of the distributed estimation by subscribing the noise estimation service in different subscription frequencies $f_{sub}$ at edge is shown in  Fig.~\ref{fig:dist_est}, where the $f_{sub}$ is $0~Hz$ means no subscription. The frequency of simulation $f_{sim}$ and sensor data uploading $f_{upl}$ are both $10~Hz$.

The first row in Fig.~\ref{fig:dist_est} shows the mean of MSE of the distributed estimation in all CAVs with respect to ground truth with three wireless communication ranges in V2X environment, where the scenario $0~m$ radius indicates the improvement of local perception by receiving the estimated noise value of local OBS from edge. As expected, the higher $f_{sub}$ speeds up the convergence speed of distributed estimation, although the different between $10Hz$ and $1Hz$ is pretty small. However, the results shows a remarkable improvement by subscribing the noise estimation service comparing with no subscription. The second row, where the mean of MSE of the distributed estimation in all CAVs with respect to the estimation limit that uses noise ground truth for distributed estimation, also proves the subscription can strongly enhance the distributed estimation, in order to increase the accuracy approach the limit. We define the improvement rate by mean of ${(\varepsilon-\varepsilon^{*})}/{\varepsilon}$ and the simulation shows the distributed estimation to the ground truth is improved over $80\%$\ and the to the estimation limit is improved around $99.5\%$,  In another word, the distributed estimation by subscribing the BiFNoE based noise estimation service is nearly the same as the estimation with true noise values.

%By taking the received noises into the distributed data fusion, the MSE reduces after $5~s$ from $3~m$ down to around $0.1~m$. The mean of estimation results in the vehicle fleet is improved over $80\%$, which is acquired by mean of ${(\varepsilon-\varepsilon^*)}/{\varepsilon}$. The MSE of estimation with noise learning with respect to the limit of distributed data fusion, which estimates the targets based on noise ground truth, is shown in figure~\ref{fig:dst_target_est_2}. The estimation is improved around $99.5\%$, which is nearly the same as the estimation with true noises.

\subsection{Carla Simulation \Crs{(to be done for protocol evaluation}}

In order to evaluate our method in consideration of road topology, enriched traffic environment, vehicle dynamics, sensor perception models from raw data to object tracking, we demonstrate the BiFNoE and noise estimation service in CARLA simulation \cite{dosovitskiy2017carla} with 50 CAVs and 50 normal vehicles, which is similar like the applied scenario in \cite{Shorinwa2020}. 

\subsection{Protocol Evaluation \Crs{(to be rewritten after Carla simulation, first test has been finished by cooperation with Numan))}}

To evaluate the performance of the protocol, we investigate how a varied update rate $f_{upd}$ at the edge server can affect the results of noise estimation and performance of centralized as well as distributed data fusion. Due to the limited bandwidth, the edge server can not acquire the object lists from all CAVs with the same frequency. Though a lower update rate causes the decreasing of the estimation accuracy in some extent, the requirement on communication performance, such as bandwidth, latency can be significantly reduced. Furthermore, the change of the noise values in a short time duration can be ignored. The delay from computation at edge and data transmission from edge server to CAVs do not influence the enhancement in distributed data fusion.

\begin{figure}[ht]
\includegraphics[width=0.49\textwidth]{figures/improvement_rate.PNG}
\caption{Improvement Rate of Our Protocol and Direct Sharing Centralized Estimation with Noise Estimation in Different Update Frequency at Edge Server}
\label{fig:ProtocolEvaluation}
\end{figure}

Fig.~\ref{fig:ProtocolEvaluation} shows the improvement rate of our protocol and direct sharing centralized estimations with noise estimations in different update frequency at edge. Directly sharing results of centralized data fusion with algorithm~\ref{alg:BiFNoE} in frequency of $50~Hz$ can improve the perception accuracy at each vehicle up to $90\%$, however in low frequency, e.g. in $1~Hz$, the accuracy can be even reduced, because of lacking of estimation update. The latency of the data transmission will further decrease the quality of estimation results. In contrast, our proposed protocol, which only sends the noise values to each vehicle, is insensitive to the changes of update rate and can improve the distributed perception over 
$80\%$ in $2~s$. When the extended \emph{SENSORIS} is used for our protocol, only $11.3~kbps$ 
downlink bit rate can archive the similar perception accuracy at each vehicle instead of at least $113.6~kbps$ using directly sharing.

\begin{comment}
\begin{table*}[ht]
\begin{threeparttable}
\caption{\centering Overview of Communication Performance Requirement and Estimation Improvement with Different Centralized Update Rate at edge Server}
\label{table:V2X}
\centering
\begin{tabular}{C{2cm}C{2cm}C{2cm}C{2cm}C{2cm}C{2cm}C{2cm}C{2cm}}
\toprule %%%%%%%%%%%%%%%%%%
   \textbf{Update Rate (Hz)} & \textbf{$f_{bdc}:f_{upl}$} & \textbf{UL Bit Rate (kbps)} & \textbf{DL Bit Rate (kbps)} & \textbf{MSE Noise Est. ($m^2$)} & \textbf{MSE Dst. Est. ($m^2$)} & \textbf{Imp. Rate \newline{(\%)}} \\ 
\midrule %%%%%%%%%%%%%%%%%%
   $50$ & $1:1$ &  & $571.2$ & & &$97.20$\\
   $10$ & $5:1$ &  & $113.6$ & && $97.63$\\
   $1$ & $50:1$ &  & $11.3$ & &&$97.12$\\
\bottomrule  %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table*}
\end{comment}
